On the dynamical Lie algebras of quantum approximate optimization algorithms

Dynamical Lie algebras (DLAs) have emerged as a valuable tool in the study of parameterized quantum circuits, helping to characterize both their expressiveness and trainability. In particular, the absence or presence of barren plateaus (BPs) -- flat regions in parameter space that prevent the efficient training of variational quantum algorithms -- has recently been shown to be intimately related to quantities derived from the associated DLA. In this work, we investigate DLAs for the quantum approximate optimization algorithm (QAOA), one of the most studied variational quantum algorithms for solving graph MaxCut and other combinatorial optimization problems. While DLAs for QAOA circuits have been studied before, existing results have either been based on numerical evidence, or else correspond to DLA generators specifically chosen to be universal for quantum computation on a subspace of states. We initiate an analytical study of barren plateaus and other statistics of QAOA algorithms, and give bounds on the dimensions of the corresponding DLAs and their centers for general graphs. We then focus on the $n$-vertex cycle and complete graphs. For the cycle graph we give an explicit basis, identify its decomposition into the direct sum of a $2$-dimensional center and a semisimple component isomorphic to $n-1$ copies of $su(2)$. We give an explicit basis for this isomorphism, and a closed-form expression for the variance of the cost function, proving the absence of BPs. For the complete graph we prove that the dimension of the DLA is $O(n^3)$ and give an explicit basis for the DLA.

==> DLA-journal-prelim.tex <==
For two sets $T_1$ and $T_2$, $T_1-T_2\defeq \{t: ~t\in T_1,~t\notin T_2\}$. For any integer $n$, let $[n]\defeq\{1,2,\ldots,n\}$, and define the parity function $\parity(n)=1$ if $n$ is odd and $\parity(n)=0$ if $n$ is even. {For any $A,B\in \mbC^{n\times n}$, their Hilbert–Schmidt inner product is defined as $\langle A,B\rangle \defeq \tr(A^\dagger B)$. For a subspace $W$ of a vector space $V$, we denote by $\Pi_W$ the orthogonal projection onto $W$. $S_n$ denotes the symmetric group on $n$-elements.} 



We denote $n$-qubit Pauli strings by $P=P_1P_2\cdots P_n \defeq P_1\otimes P_2\otimes\cdots \otimes P_n$, where $P_j\in\{I,X,Y,Z\}$, $I$ is the $2\times 2$ identity matrix, and 
\eq{
X &=  \begin{pmatrix} 0 & 1 \\ 1 & 0\end{pmatrix}, 
\quad Y = \begin{pmatrix} 0 & -i \\ i & 0\end{pmatrix}, 
\quad Z = \begin{pmatrix} 1 & 0 \\ 0 & -1\end{pmatrix}
}
are the standard Pauli operators. The set of all $n$-qubit Pauli strings is denoted $\+P_n$. Subscripts indicate the qubit number that a Pauli operator (or identity) acts on, e.g., $X_1 Y_2 Z_3 I_4 I_5$ means to apply $X$, $Y$ and $Z$ on the first, the second and the third qubits, respectively. Identity operators may sometimes be dropped, e.g.,  we may simply write $X_1 Y_2 Z_3$ for $X_1 Y_2 Z_3 I_4 I_5$. We use $P_{-j}$ to denote Pauli strings indexed by $[n]- \{j\}$. Note that for a Pauli string $P=P_1P_2\cdots P_n$, we have $[P,\sum_{j=1}^n X_j] = \sum_{j=1}^n ([P_j, X_j] \otimes P_{-j}) = \sum_{j=1}^n Q_j\otimes P_{-j}$, where $Q_j = 0$ if and only if $P_j = X_j$ or $I_j$.  

The following lemmas on basic algebra will be useful:
% \begin{lem}[Vieta's formulas, \cite{coolidge2004treatise}]\label{lem:vieta} Let $P(x)=\sum_{j=0}^n a_j x^j$ be a degree-$n$ polynomial with coefficients $a_j\in\mb{C}$, and let $z_1, \ldots, z_n\in\mb{C}$ be the roots of $P$. Then, for $1\le k \le n$,
% \eq{
% (-1)^{k}a_{n-k}/a_n&=\sigma_k(z_1, \ldots, z_n),
% }
% where $\sigma_k(z_1, \ldots, z_n)\defeq \sum_{1\le j_1<j_2<\cdots < j_k\le n}z_{j_1}z_{j_2}\cdots z_{j_k}$ is the elementary symmetric polynomial of degree $k$.
% \end{lem}

% \begin{lem}[Cayley-Hamilton theorem, \cite{mirsky2012introduction}]\label{lem:cayley-ham} Let $A\in\mb{C}^{n\times n}$ be a square matrix, and $p_A(\lambda) = \det(\lambda I-A)$ its characteristic polynomial. Then $p_A(A) = 0$.
% \end{lem}

% \begin{lem}[Inverse of Vandermonde matrix, \cite{rawashdeh2019simple}]\label{eq:inverse-vandermonde}
%     Let $\lambda_1,\lambda_2,\cdots, \lambda_{n}$ be distinct real numbers and $\Lambda=[\Lambda_{km}]\in \mbR^{n\times n}$  with $\Lambda_{km}=\lambda_m^{k-1}$ be the Vandermonde matrix. Then the inverse of $\Lambda$ is the matrix whose elements are
%     \[(\Lambda^{-1})_{km}=(-1)^{n-m} \frac{\sigma_{n-m}(\lambda_{[n]-k})}
%     {\prod_{1 \leq j \leq n, j\neq k} (\lambda_k - \lambda_j)},\]
%     where $ \lambda_{[n]-k}= \lambda_{1}, \ldots,
%     \lambda_{k-1}, \lambda_{k+1}, \ldots , \lambda_{n}$, $\sigma_0(\lambda_{[n]-k})\defeq 1$ and $\sigma_j(\lambda_{[n]-k})$ is the elementary symmetric polynomial of degree $j$ for $j\ge 1$.
% \end{lem}

\subsection{Lie algebra}

Here we review a number of basic facts about Lie algebras; see \cite{hall2013lie} or \cite{knapp1996lie}, for instance, for a more comprehensive introduction to the topic.  

    A Lie algebra $\.g$ is a vector space $V$ over a field $\mbF$ together with a bilinear map  $[\cdot,\cdot]:\.g\times \.g \to \.g$, called the \textit{Lie bracket}, satisfying (1) $[A,A] = 0$ for all $A\in \.g$, and (2) Jacobi identity  
    \begin{align} \label{eq:Jacobi}
        [A,[B,C]] + [B,[C,A]] + [C,[A,B]] = 0, \quad \forall A,B,C\in \.g. 
    \end{align} 
If $[A,B]=0$ for all $A,B\in\.g$ then $\.g$ is said to be  \emph{commutative}. A \emph{Lie subalgebra} $\.h\subseteq\.g$ of a Lie algebra $\.g$ is a linear subspace of $\.g$ which is closed under the Lie bracket, i.e. $[H_1,H_2]\in \.h$ for all $H_1, H_2\in \.h$.  A Lie algebra is said to be \emph{compact} if it is the Lie algebra of a compact Lie group (see \cite{hall2013lie} or \cite{knapp1996lie} for further details). 

In this paper we will mainly be concerned with matrix Lie algebras, where the elements of $\.g$ are matrices, and for which the Lie bracket is the commutator $[A,B] = AB-BA$. If $\.g$ is a real matrix Lie algebra with basis elements $\{E_1, E_2, \ldots, E_N\}$ that are independent over $\mb{C}$, the \emph{complexification} of $\.g$, denote $\.g_\mb{C}$, is defined to be the complex matrix Lie algebra
\eq{
\.g_\mb{C}&= \spn_\mb{C}\{E_1, \ldots, E_n\}.
}
A number of matrix Lie algebras that will be used in this paper are listed below.
\begin{enumerate}
    \item $\.{sl}(n,\mbF) \defeq \{H\in \mbF^{n\times n}: \tr(H) = 0\}$, which has dimension $n^2-1$.
    
    \item $\.{so}(n,\mbC) \defeq \{H\in \mbC^{n\times n}: H^T = -H\}$, which has dimension $n(n-1)/2$.
    
    \item $\.{sp}(n,\mbC) \defeq \{H\in \mbC^{2n\times 2n}: \Omega H + H^T \Omega = 0\}$ for $\Omega \defeq \begin{bmatrix}
        0 & I_n \\ I_n & 0
    \end{bmatrix}$, which has dimension $n(2n+1)$.

    \item $\.{u}(n) \defeq\{H\in \mbC^{n\times n}: H^\dagger = -H\}$, which has dimension $n^2$.
    
    \item $\.{su}(n) \defeq \{H\in \mbC^{n\times n}: H^\dagger = -H, \tr(H) = 0\}$, which has dimension $n^2-1$.
\end{enumerate}
A Lie algebra $\.g$ is said to be the direct sum of subalgebras $\.g_1, \.g_2, \ldots, \.g_k$, denoted
\eq{\.g = \.g_1 \oplus \.g_2 \oplus \ldots \oplus \.g_k,}
    if it is the direct sum of $\.g_1, \ldots, \.g_k$ as vector spaces, and $[\.g_i, \.g_j] = 0$ for all $i\neq j$. An \textit{ideal} of a Lie algebra $\.g$ is a Lie subalgebra $\.i$ of $\.g$ satisfying the further requirement that $[A,B]\in \.i$ for all $A\in \.g$ and $B\in\.i$. An ideal $\.i$ of $\.g$ is \textit{trivial} if $\.i = \.g$ or $\.i = 0$. For any $\.g$, one can define the following two ideals:
\eq{
Z(\.g) &\defeq \{ A\in \.g : [A,B]=0, \forall \,B\in \.g\}, &\quad (\text{center of }\.g) \\
[\.g, \.g]&\defeq \spn\{[A,B] : A, B\in\.g\},&\quad (\text{commutator ideal}) 
}
A \textit{simple Lie algebra} is a Lie algebra that is non-abelian and contains no nontrivial ideals. A \textit{semisimple Lie algebra} is one which is the direct sum of simple Lie algebras. Given a Lie algebra $\.g$ and any $A\in \.g$, the associated \textit{adjoint map} is the linear transformation $ad_A:\.g\ra \.g$ given by $ad_A(B) = [A,B]$.    A \emph{Cartan subalgebra} $\.h\subseteq\.g$ of a complex semisimple Lie algebra is a maximal commutative subalgebra of $\.g$, where $ad_H$ is diagonalizable for all $H\in\.h$.

The following theorems will be useful in subsequent sections.
\begin{thm}[\cite{knapp1996lie}]\label{thm:cartan-conjugate} Let $\.g$ be a complex semisimple Lie algebra, and let $Aut(\.g)$ denote the automorphism group of $\.g$, i.e., the set of bijective linear maps $\phi:\.g\ra\.g$ such that $[\phi(A), \phi(B)] = \phi([A,B])$. If $\.h_1, \.h_2$ are Cartan subalgebras of $\.g$, there exists $\phi\in Aut(\.g)$ such that $\phi(\.h_1)=\.h_2$.
\end{thm}

\begin{thm}[\cite{erdmann2006introduction}]\label{fact:adh-diagonalizable} Let $\.g$ be a matrix Lie algebra over $\mb{C}$ or $\mb{R}$. If $H\in\.g$ is diagonalizable then $ad_H:\.g\ra\.g$ is diagonalizable. 
\end{thm}



% \begin{lem}[\rm\cite{hota2014real}]\label{lem:sl2c-complexification}
% $\.{sl}(2,\mbR)_\mbC = \.{su}(2)_\mbC = \.{sl}(2,\mbC)$, and the only real Lie algebras whose complexification is $\.{sl}(2,\mbC)$ are $\.{sl}(2,\mbR)$ (non-compact) and  $\.{su}(2)$ (compact).
% \end{lem}

\begin{thm}[\cite{knapp1996lie}]
    Any subalgebra $\.g$ of $\.{sl}(n,\mbF)$, where $\mbF = \mbR$ or $\mbC$, has the following decomposition 
    \begin{align}
        \.g = \.c \oplus \.g_1 \oplus \cdots \oplus \.g_k
    \end{align}
    where $\.c = Z(\.g)$ is the center of $\.g$, and each $\.g_j$ is a simple Lie algebra over $\mbF$. 
\end{thm}
Note that, if $\.g$ has the above decomposition $\.g = \.c\oplus \.g_1\oplus\ldots \oplus\.g_k$, then $[\.g,\.g] = \.g_1\oplus\ldots \oplus\.g_k$ and is semisimple.



% \begin{thm}[\cite{hall2013lie}]\label{thm:classification}
%     Every finite-dimensional simple Lie algebra over $\mathbb{C}$ is isomorphic to precisely one of the following.
%     \begin{enumerate}
%         \item $A_n=\.{sl}(n+1,\mathbb{C})$ for $n\ge 1$, with dimension $n^2+2n$;
%         \item $B_n=\.{so}(2n+1,\mathbb{C})$ for $n\ge 2$, with dimension $2n^2+n$;
%         \item $C_n=\.{sp}(n,\mathbb{C})$ for $n\ge 3$, with dimension $2n^2+n$;
%         \item $D_n=\.{so}(2n,\mathbb{C})$ for $n\ge 4$, with dimension $2n^2-n$;
%         \item The ``exceptional'' Lie algebras $G_2$, with dimension $14$; $F_4$, with dimension $52$; $E_6$, with dimension $78$; $E_7$, with dimension $133$; and $E_8$, with dimension $248$. 
%     \end{enumerate}
%     The dimensions of Cartan subalgebras of $A_n$, $B_n$, $C_n$, and $D_n$ are $n$, while those of $G_2$, $F_4$, and $E_j$ are $2$, $4$, and $j$ respectively, for any $j\in \{6,7,8\}$.
% \end{thm}

\subsection{Dynamical Lie algebras}


We focus in this paper on the Lie algebras corresponding to layered PQCs.

\begin{defi}[Dynamical Lie algebra (DLA)]\label{def:dla} Let $U$ be a layered parameterized quantum circuit (see Eq.~\eqref{eq:pqc}) with a set $\+A=\{iH_1, \ldots, iH_s\}$ of \emph{DLA generators}. The corresponding DLA, denoted
\eq{
\.g&=\langle\+A\rangle_{\text{Lie}, \mbR},
}
is the Lie algebra (over $\mbR$), with $[A,B]\defeq AB-BA$, spanned by all possible nested commutators of elements in $\+A$.
\end{defi}

Note that, due to the Jacobi identity, we can assume without loss of generality that all nested commutators are of the form $[H_1, [H_2, [ \ldots, H_s]]]$. 
\begin{defi}[Degree of a DLA] Let $\langle \+A\rangle_{\text{Lie},\mb{F}}$ be a dynamical Lie algebra. Its degree $\operatorname{Deg}(\langle \+A\rangle_{\text{Lie},\mb{F}})$ is the smallest integer $d$ such that any $X\in\langle \+A\rangle_{\text{Lie},\mb{F}}$ can be expressed as a linear combination of $d$-layered nested commutators $[H_1, [H_2, [ \ldots, [H_d,H_{d+1}]\ldots ]]]$. 
\end{defi}

% Algorithm~\ref{alg:DLA-generation} gives a procedure for computing a basis for a DLA (and hence its dimension) and computing its degree from its set of generators.

% \begin{algorithm}[!htb]
%     \caption{Generate DLA}
%     \label{alg:DLA-generation}
%     \textbf{Input}: a set of elements $\+A = \{H_1, \ldots, H_s\}$ in a finite-dimensional Lie algebra $\.g$ over field $\mbF$.\\
%     \textbf{Output}: $(\+B,k)$, where $\+B$ is a basis of $\langle \+A \rangle_{\text{Lie},\mbF}$, i.e. $\langle \+A \rangle_{\text{Lie},\mbF} = \spn_{\mbF}\{H: H\in \+B\}$, and $k=\operatorname{Deg}(\langle \+A\rangle_{\text{Lie},\mb{F}})$.\\  %level of the generation.\\
%     \begin{algorithmic}[1]
%         \STATE Let $\+B_0$ be a maximal subset of linearly independent elements from  $\+H$
%         \STATE $V_0 := \spn_{\mbF} \{H: H\in \+B_0\}$
%         \FOR{ $k = 1, 2, \ldots$ }
%         \STATE $\+B_k := \+B_{k-1}$, $V_k:= V_{k-1}$
%             \FOR{$H^{(0)}\in \+B_{0}$} 
%                 \FOR{ $H^{(k-1)}\in \+B_{k-1} - \+B_{k-2}$}
%                 \STATE compute $H = [H^{(0)}, H^{(k-1)}]$
%                 \IF{ $H\notin V_k$}
%                     \STATE  let $\+B_k := \+B_{k-1}\cup \{H\}$ and $V_k:= \spn_{\mbF} \{V_k,H\}$
%                 \ENDIF
%                 \ENDFOR
%             \ENDFOR
%             \IF{$\+B_k = \+B_{k-1}$}
%                 \STATE  return $(\+B_k,k-1)$
%             \ENDIF
%         \ENDFOR
%     \end{algorithmic}
% \end{algorithm}

\begin{defi}[$\.g$-purity]
    The $\.g$-purity of a Hermitian operator $H$ is 
    \[\+P_{\.g}(H)\defeq\tr(H_{\.g}^2)=\sum_{j=1}^{\dim(\.g)}|\tr(E_j^\dag H)|^2,\]
    where $H_\.g$ is the orthogonal (with respect to Hilbert-Schmidt inner product $\langle A,B\rangle \defeq \tr (A^\dag B)$) projection of operator $H$ onto $\.g_{\mbC}$, and $\{E_j: j=1,2,\ldots,\dim(\.g)\}$ is an orthonormal basis for $\.g$. 
\end{defi}
The following important result relates the expectation and variance of the loss function to the DLA. A parameterized circuit $U(\theta)$ is a \textit{unitary 2-design} if 
\[
    \int_{\theta} U(\theta)^{\otimes 2} \otimes (U(\theta)^*)^{\otimes 2} d\theta = \int_{U} U^{\otimes 2} \otimes (U^*)^{\otimes 2} dU
\]
where the left integral is over uniform distribution of $\theta$ and the right integral is over the Haar measure of all $n$-qubit unitary $U$. It is known that an $L$-layered quantum circuit $U_L(\theta_L)U_{L-1}(\theta_{L-1})\cdots U_1(\theta_1)$ with $U_\ell(\theta_\ell) = \prod_{k=1}^K e^{-iH_k \theta_{\ell,k}}$ is an $\epsilon$-approximate 2-design, with $\epsilon$ decreasing exponentially in $L$ \cite{ragone2023unified}.

\begin{thm}[\cite{ragone2023unified}]\label{thm:dla-var-purity} Let $\.g=\.c\oplus \.g_1 \oplus \ldots \oplus \.g_k$ be the DLA of a variational quantum algorithm. If (1) $O\in i\.g$ or $\rho\in i\.g$, and (2) the circuit is a unitary 2-design, then
\eq{
\av_\theta[\ell(\rho,O;\theta)] &= \tr(\rho_{\.c}O_{\.c}), \quad 
\var_\theta[\ell(\rho,O;\theta)] = \sum_{j=1}^k \frac{\mcP_{\.g_j}(\rho) \mcP_{\.g_j}(O)}{\dim(\.g_j)}.
}
\end{thm}
% Note that the dimension of $\.g$ alone is not sufficient for giving non-trivial lower-bounds on the variance, as the purities of $\rho$ and $O$ may distribute on different subspaces $\.g_j$, in which case the variance can be 0. Therefore, lower bounding the variance requires understanding the decomposition of the Lie algebra into simple subalgebras, and how the purities distribute amongst these subalgebras.





